AnySat: One Earth Observation Model for Many Resolutions, Scales, and Modalities

Geospatial models must adapt to the diversity of Earth observation data in terms of resolutions, scales, and modalities. However, existing approaches expect fixed input configurations, which limits their practical applicability. We propose AnySat, a multimodal model based on joint embedding predictive architecture (JEPA) and scale-adaptive spatial encoders, allowing us to train a single model on highly heterogeneous data in a self-supervised manner. To demonstrate the advantages of this unified approach, we compile GeoPlex, a collection of 5 multimodal datasets with varying characteristics and $11$ distinct sensors. We then train a single powerful model on these diverse datasets simultaneously. Once fine-tuned or probed, we reach state-of-the-art results on the test sets of GeoPlex and for 6 external datasets across various environment monitoring tasks: land cover mapping, tree species identification, crop type classification, change detection, climate type classification, and segmentation of flood, burn scar, and deforestation. The code and models are available at https://github.com/gastruc/AnySat.

==> 2_related_bk.tex <==
%auto-ignore
\paragraph{Self supervised Learning and feature predictive architecture}

Self-Supervised learning consists in learning expressive data representations without labels by using a pretext task. This approach has been particularly successful for pertaining image analysis models. These approaches can be divided into contrastive ones based on minimizing the distance between representations of paired samples \cite{chen2020simple,he2020momentum} and generative ones based on the reconstruction of an image based on a degraded version of it \cite{dosovitskiy2020image,he2022masked}. 
Some methods such as data2vec \cite{baevski2022data2vec} and ConMIM \cite{yi2023masked} learn to reconstruct a signal in latent space directly.
However, recent work has shown that feature prediction can be used as self-supervised signal instead of pixel or embedding reconstruction. 
It is the case of Joint-Embedding Predictive Architecture (JEPA) \cite{assran2023self}, which learns to predict the embeddings of a part of an image signal from an overlapping part of it and by comparing it to the embedding of the corresponding part.
JEPA is based on a teacher-student training scheme and a multi-block masking strategy without unnecessary pixel-level details. 
JEPA pre-training is computationally efficient because it does not require intensive multiview data augmentations and is decoder free.
JEPA provides strong off-the-shelf semantic representations and is competitive with other self-supervised pertaining methods \cite{assran2023self}.
Latent MIM \cite{wei2024towards} combines a scheme similar to JEPA with a contrastive loss to learn more diverse representations in the image.%JEPA like + contrastif:

\paragraph{Self supervised on Geospatial data.}

Self-supervised learning has recently thrived in the geospatial domain due to the abundance of available data.
Contrastive approaches have been successfully adapted to EO, for which samples are paired according to their location \cite{tseng2022croco} or the time of acquisition \cite{ayush2021geography,manas2021seasonal}.
%Papiers qui reconstruisent en pixel space:
%This principle has been successfully adapted to EO analysis \cite{gao2022general,cong2022satmae,yuan2022sits}, and was further extended to handle multiple spatial scales \cite{reed2023scale},  multimodality \cite{fuller2023croma,irvin2023usat}, or hyperspectral observations \cite{ibanez2022masked,liu2022band}.
Generative model has been successfully adapted to EO analysis \cite{gao2022general,cong2022satmae,yuan2022sits,wang2022ssl4eo,jakubik2310foundation}. Most of the methods adapted to EO, the Masked Auto Encoder (MAE) paradigm \cite{he2022masked} by reconstructing a degraded version of the image in pixel space as supervision signal. 
Some methods add masking on the spectral \cite{cong2022satmae} or temporal dimension \cite{yuan2022sits}, angle variation \cite{li2024masked}, multi-scale training \cite{noman2024rethinking,tang2024cross}, 3D spatio-temporal positional encoding \cite{jakubik2310foundation} or metadata supervision \cite{bourcier2024learning}.
ScaleMAE \cite{reed2023scale} introduces a ground sample distance-based positional encoding to deal with the scale information present in remote sensing data and help to generalize at unseen scale but only for a single image. 
The Prithvi model \cite{jakubik2310foundation} trained with MAE on Landsat 8-9 and Sentinel-2 images effectively transferred \cite{hsu2024geospatial} to VHR image or strongly different sensor such as THEMIS, but is limited to six spectral band and single-date image.
U-BARN \cite{dumeur2024self} and ALISE \cite{dumeur2024paving} applied this MAE paradigm to time series.
Note that several methods mixed constrastive and generative methods such as \cite{tang2024cross,fuller2023croma}.
%, and was further extended to handle multiple spatial scales \cite{reed2023scale}.
%,  multimodality \cite{fuller2023croma,irvin2023usat}, or
%hyperspectral observations \cite{ibanez2022masked,liu2022band}.
%SatMAE \cite{cong2022satmae} utilized the mask image modeling for multi-spectral, temporal and optical remote sensing data. 



%\cite{cong2022satmae} \cite{reed2023scale} 
%\cite{noman2024rethinking} 
%\cite{li2024s2mae} 
%\cite{li2024masked} 
%\cite{tang2024cross}
%\cite{wang2022ssl4eo}

%prithvi analysis : \cite{hsu2024geospatial} : pixel space with multiple sensor (aerial mono temporal)
%prithvi : \cite{jakubik2310foundation}

%reconstruction en latent space: 
On the other hand, few methods tend to reconstruct in latent space. SAR-JEPA \cite{li2024predicting} applies a Joint-Embedding Predictive Architecture to SAR image, outperforming MAE based methods for classification task.

%Papiers qui utilisent plusieurs modalités alignées:

Multimodal learning also has a long history in EO due to the large variety and complementarity of sensors \cite{ghamisi2019multisource}. In self-supervised learning, the spatial alignment of modalities serves mainly as the supervision signal but most of the proposed methods are limited to single image and required a specific encoder per modality or scale. 
CROMA \cite{fuller2023croma}, MMEarth\cite{nedungadi2024mmearth} and MultiSSL \cite{xue2025multimodal} are specifically designed for paired optical and radar observations, but cannot handle Very High Resolution (VHR) data. USat \cite{irvin2023usat} considers mono temporal images with different resolutions.
msGFM \cite{han2024bridging}, USat \cite{irvin2023usat} and CROMA \cite{fuller2023croma}  require one patch embedding and decoder per modality while sharing the encoder among them. 
DOFA with a wavelength-conditioned patch embedding is able to share its backbone across modalities and to deal with a variable number of spectral bands but it can only process single-image. 
%but only takes a single date within a time series.


%\cite{irvin2023usat} \cite{fuller2023croma} 
%\cite{nedungadi2024mmearth} 
%\cite{xiong2024dofa}
%msGFM : \cite{han2024bridging}
%\cite{xue2025multimodal}

%Papiers qui utilisent différentes modalités et potentiellement des time series aussi:
More recent works propose to tackle together time series and high-resolution single images to take advantage of the complementary of high temporal resolution and high spatial resolution data. SatlasNet \cite{bastani2023satlaspretrain} encodes each image independently before applying a temporal max polling on them destroying all the signal's temporal information. 
SkySense \cite{guo2024skysense} pre-training is based on a teacher-student structure and region-specific prototype used in an attention mechanic.
OmniSat \cite{astruc2024omnisat} is based on MAE-style training mixed with constrastive loss to learn latent token combining information from the different modalities.
However, they all need to train a specific encoder per modality \cite{astruc2024omnisat,guo2024skysense,bastani2023satlaspretrain} in contrast to our method. 

%\cite{astruc2024omnisat} 
%\cite{dumeur2024paving} 
%\cite{guo2024skysense} : supervise by prototy per area on the globe


% CCL 
DOFA \cite{xiong2024dofa} uniquely processes novel frequencies, ScaleMAE and follow-ups \cite{reed2023scale,noman2024rethinking,tang2024cross} handles unseen resolutions, OmniSat \cite{astruc2024omnisat} accommodates time sequences of any size, on the contrary, our proposed method can handle different resolutions, scales, and sensor types. 

==> figures/training.tex <==
\includegraphics[width=1\linewidth]{example-image}

==> tables/linear.tex <==
\begin{tabular}{l l c}\toprule
     & Pretrain Data & mIoU \\\midrule
     \bf AnySat (ours) & S2NAIP & \\
     \bf AnySat (ours) & FLAIR & \\ 
     \bf AnySat (ours) & GeoPlex & \\\greyrule
  ScaleMAE \cite{reed2023scale} & FMoW \cite{christie2018functional} & 51.9 \\
  XSTARS \cite{marsocci2024cross} & S2-LS \cite{marsocci2024cross} & 48.1\\
  SatMAE \cite{cong2022satmae} & FMoW-Sentinel \cite{christie2018functional,cong2022satmae} & 46.7 \\
\end{tabular}

==> tables/treesat.tex <==
\resizebox{\linewidth}{!}{
\begin{tabular}{ll cc cc cc cc}
\toprule
\multirow{2}{*}{Model} & pre- &  \multicolumn{2}{c}{~\hspace{6mm} \bf All \hspace{6mm}~ } & \multicolumn{2}{c}{ ~\hspace{1mm} Sentinel-1 \hspace{1mm}~ } & \multicolumn{2}{c}{~\hspace{1mm} Sentinel-2 \hspace{1mm}~} & \multicolumn{2}{c}{~\hspace{1mm} VHR Image \hspace{1mm}~} \\\cmidrule(r{4pt}){3-4} \cmidrule(r{4pt}){5-6} \cmidrule(r{4pt}){7-8} \cmidrule(r{4pt}){9-10}
& {training\hspace{5mm}~}& 10\% & 100\% & 10\% & 100\% & 10\% & 100\% & 10\% & 100\%\\
\midrule
  DOFA \cite{xiong2024dofa} & \;\;\globe & 41.8\deadstar & 71.3\deadstar & 0.0 & 0.0 & 25.0 & 39.4 & 51.6 & 67.5 \\
  OmniSat \cite{astruc2024omnisat} & TSAI-TS & 61.1 & 74.2 & 48.2 & 56.7 & 51.4 & 62.9 & 58.3 & 70.5 \\
  AnySat (ours) & No & 52.4 & 73.8 & 29.1 & 54.1 & 42.8 & 70.0 & 47.1 & 68.5 \\
  \bf AnySat (ours) & Pile &  &  &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
